Multitask Identity-Aware Image Steganography via Minimax Optimization

High-capacity image steganography, aimed at concealing a secret image in a cover image, is a technique to preserve sensitive data, e.g., faces and fingerprints. Previous methods focus on the security during transmission and subsequently run a risk of privacy leakage after the restoration of secret images at the receiving end. To address this issue, we propose a framework, called Multitask Identity-Aware Image Steganography (MIAIS), to achieve direct recognition on container images without restoring secret images. The key issue of the direct recognition is to preserve identity information of secret images into container images and make container images look similar to cover images at the same time. Thus, we introduce a simple content loss to preserve the identity information, and design a minimax optimization to deal with the contradictory aspects. We demonstrate that the robustness results can be transferred across different cover datasets. In order to be flexible for the secret image restoration in some cases, we incorporate an optional restoration network into our method, providing a multitask framework. The experiments under the multitask scenario show the effectiveness of our framework compared with other visual information hiding methods and state-of-the-art high-capacity image steganography methods.

==> revision/comp_steg_other_high_PSNR.tex <==

\begin{table*}[h]
	\centering
	\caption[TABLE]{Comparison with State-of-the-Art High-Capacity Image Steganography Methods on the AFD Dataset.
	$\uparrow$ means the higher the better; $\downarrow$ means the lower the better.
	}
	% \begin{center} 
	%\resizebox{\textwidth}{!}{%
		\label{Table_Comparison_Steganography_high_PSNR} 
		%  \makebox[\textwidth][c]{
		\begin{tabular}{lcccccccc}
			\toprule
			 \multirow{2}{*}{ \textbf{Model}} & \multicolumn{3}{c}{ \textbf{Cover-Container}}                        & \multicolumn{3}{c}{ \textbf{Secret-Restored}}                       & \multirow{2}{*}{Acc$\uparrow$}& \multirow{2}{*}{Original Acc$\uparrow$} \\ \cmidrule(lr){2-4}\cmidrule(lr){5-7}
			& MSE$\downarrow$               & PSNR$\uparrow$               & MS-SSIM$\uparrow$            & MSE$\downarrow$               & PSNR$\uparrow$               & MS-SSIM$\uparrow$            &                     &                      \\  \toprule
			 HliPS* & 0.0012 & 29.35 & 0.9687 & 0.0014 & 28.54 & 0.9808  & 0.6195 & 0.8177 \\
			 SteganoGAN* & 0.0114 & 19.42 & 0.9484 & 0.0449 & 13.47 & 0.8665  & 0.5282 & 0.8473 \\
			 HiDDeN* & 0.0011 & 29.59 & \textbf{0.9850} & 0.0070 & 21.55 & 0.9239  & 0.6705 & 0.8373 \\
			 StegNet* & 0.0019 & 27.28 & 0.9733 & 0.0066 & 21.78 & 0.9524 & 0.4990 & 0.8493 \\
			 Ours & \textbf{0.0010} & \textbf{30.09} & 0.9849 & \textbf{0.0007} & \textbf{31.37} & \textbf{0.9811} & \textbf{0.7955} & 0.8690 \\ \toprule
		\end{tabular}
	%}
\end{table*}

==> revision/deep_steganalysis.tex <==
\begin{table*}[htbp]
    \caption{The neural steganalysis results. Both the two cases are trained with 4000 image pairs, and tested on 1000 image pairs. In the first case, training data consists of the same specific steganography method. In the second case, the training data consists of the other four methods evenly, which is called leave-one-subject-out cross-validation from the perspective of steganography method.}
    \centering
    \begin{tabular}{lcccccccc}
        \toprule
%        \multicolumn{2}{c}{First case} & \multicolumn{2}{c}{Second case}\\ 
%        \cline{1-2} \cline{3-4} 
		& \textbf{Publication} & \textbf{Year}
        & \textbf{Model} & \textbf{HiDDeN} & \textbf{HliPS} & \textbf{SteganoGAN} & \textbf{StegNet} & \textbf{Ours} \\ \midrule
        \multirow{2}{*}{ \textbf{R1}} & \multirow{2}{*}{TIFS} & \multirow{2}{*}{2017}
        & First case & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\ 
        & & & Second case & 0.889 & 0.782 & 0.949 & 0.929 & 0.891 \\ \midrule
		\multirow{2}{*}{ \textbf{R2}} & \multirow{2}{*}{ICASSP} & \multirow{2}{*}{2018}
		& First case & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\ 
		& & & Second case & 0.538 & 0.613 & 0.955 & 0.690 & 0.533 \\       
%        \multirow{2}{*}{ \textbf{Model}} & \multicolumn{3}{c}{ \textbf{Cover-Container}} & \multicolumn{3}{c}{ \textbf{Secret-Restored}} & \multirow{2}{*}{DR$\downarrow$} & \multirow{2}{*}{Acc$\uparrow$} \\ 
%        \cmidrule(lr){2-4}\cmidrule(lr){5-7}
%        & MSE$\downarrow$ & PSNR$\uparrow$ & MS-SSIM$\uparrow$ & MSE$\downarrow$ & PSNR$\uparrow$ & MS-SSIM$\uparrow$ & & \\  \toprule
%        
%        Ours & 0.0012 & 29.21 & 0.9789 & 0.0005 & 33.01 & 0.9865 & 0.461 & 0.7190 \\ \toprule
        
        
        \bottomrule
    \end{tabular}
    \label{deep_steganalysis}
\end{table*}


==> revision/novelty_table.tex <==

\begin{table*}[h]
	\caption{Comparison of other steganography methods. Note that the $\mathcal{L}_{ce}$ of HiDDeN method represents the binary classification loss to indicate the cover/container image. However, in our method, the $\mathcal{L}_{ce}$ loss represents the cross-entropy loss between the container image identity and the corresponding secret image identity.
	}
	\centering
	%	\begin{center} 
	%\resizebox{\textwidth}{!}{
	\label{novelty_table} 
	%		\makebox[\textwidth][c]{
	\begin{tabular}{lcccccccccc}
		\toprule
		\multirow{2}*{\textbf{Method}} & \multirow{2}*{\textbf{Publication}} & \multirow{2}*{\textbf{Year}} & \multicolumn{3}{c}{\textbf{Task}} & \multicolumn{3}{c}{\textbf{Optimization}} \\
		\cmidrule(lr){4-6}\cmidrule(lr){7-9} & & 
		& Concealment & Restoration & Recognition 
		& $\mathcal{L}_{ce}$ & $\mathcal{L}_{cont}$ & Minimax \\
		\toprule
		HliPS [7] & NeurIPS & 2017 &$\checkmark$ & $\checkmark$ &  &   &   &   \\ 
		StegNet [50] & Future Internet & 2018 &$\checkmark$ &$\checkmark$&  &   &   \\ 
		HiDDeN [48] & ECCV & 2018 &$\checkmark$  & $\checkmark$ & & $\checkmark$ &   &   \\
		Ours & - & - &$\checkmark$ & $\checkmark$ &$\checkmark$&$\checkmark$&$\checkmark$&$\checkmark$\\
		\bottomrule
	\end{tabular}
	%	}
	%	\end{center}
\end{table*} 






==> revision/robust_cover_high_PSNR.tex <==

\begin{table*}[h]
	\caption{Robustness on Different Cover Sets with AFD Secret Set.
		$\uparrow$ means the higher the better; $\downarrow$ means the lower the better. ``100-SS'' denotes to the original 100 cover set form style transfer and satellite datasets.
	}
	\centering
	%	\begin{center} 
	%\resizebox{\textwidth}{!}{
	\label{Table_cover_robustness_high_PSNR} 
	%		\makebox[\textwidth][c]{
	\begin{tabular}{lccccc}
		\toprule
		{\textbf{Cover Set}} & MSE$\downarrow$ & PSNR$\uparrow$ & MS-SSIM$\uparrow$ & Acc$\uparrow$ & Original Acc$\uparrow$ \\
		\toprule
		100-SS &	0.0011 & 29.67 & 0.9935  & 0.8585 & 0.8752 \\
		LFW & 0.0010 & 30.07  & 0.9946  & 0.8495 & 0.8730 \\
		PASCAL-VOC12  & 0.0008 & 31.19  & 0.9953  & 0.8578 & 0.8724 \\
		ImageNet &  0.0011 & 29.65  & 0.9944  & 0.8626 & 0.8729 \\
		\bottomrule
	\end{tabular}
	%	}
	%	\end{center}
\end{table*} 





==> revision/tiny_dataset_with_restorer.tex <==

\begin{table*}[h]
	\centering
	\caption[TABLE]{Comparison with State-of-the-Art High-Capacity Image Steganography Methods on the tiny-AFD Dataset. $\uparrow$ means the higher the better; $\downarrow$ means the lower the better. The recognition accuracy (Acc) in the secret image is 0.7379.
	}
	% \begin{center} 
	%\resizebox{\textwidth}{!}{%
		\label{tiny_dataset_with_restorer} 
		%  \makebox[\textwidth][c]{
		\begin{tabular}{lcccccccc}
			\toprule
			 \multirow{2}{*}{ \textbf{Model}} & \multicolumn{3}{c}{ \textbf{Cover-Container}} & \multicolumn{3}{c}{ \textbf{Secret-Restored}}  & \multirow{2}{*}{Acc$\uparrow$}\\ 
			 \cmidrule(lr){2-4}\cmidrule(lr){5-7}
			& MSE$\downarrow$               & PSNR$\uparrow$               & MS-SSIM$\uparrow$            & MSE$\downarrow$               & PSNR$\uparrow$               & MS-SSIM$\uparrow$            &                     &                      \\  \toprule
			 HliPS* & 0.0015 & 28.36 & 0.9634 & 0.0026 & 25.88 & 0.9632 & 0.6090  \\
			 SteganoGAN* & 0.0123 & 19.09 & 0.9349 & 0.0184 & 17.36 & 0.9355 & 0.5162 \\
			 HiDDeN* & 0.0016 & 27.96 & 0.9771 & 0.069 & 21.61 & 0.9400 & 0.6522\\
			 StegNet* & 0.0024 & 26.20 & 0.9691 & 0.0070 & 21.55 & 0.9469 & 0.4855 \\
			 Ours & 0.0012 & 29.21 & 0.9789 & 0.0005 & 33.01 & 0.9865 & 0.7190\\
			 \toprule
		\end{tabular}
	%}
\end{table*}

==> revision/visual_information_table.tex <==

\begin{table*}[h]
	\caption{Clarity evaluation for different ablative container images. We adopt the variance function and Vollath function to evaluate the clarity of images. (a), (b), and (c) represent to the different examples correpsonding to \cref{ablation_visual_information_c}}
	\centering
	%	\begin{center} 
	%\resizebox{\textwidth}{!}{
	\label{visual_information_table} 
	%		\makebox[\textwidth][c]{
	\begin{tabular}{clccccc}
		\toprule
		{\textbf{Examples}} & {\textbf{Functions}} & \textbf{Cover Image} & \textbf{Baseline} & \textbf{+ $\mathcal{L}_{cont}$} & \textbf{+ Minimax} & \textbf{+ $\mathcal{L}_{cont}$ + Minimax} \\
		\toprule
		\multirow{2}{*}{(a)} 
		&Vollath$\uparrow$ & 0.2239 & 0.1975 & 0.1806 & 0.1981 & 0.1990 \\
		& Variance$\uparrow$ & 0.2087 & 0.1932 & 0.1934 & 0.1973 & 0.2072 \\
		\midrule
		\multirow{2}{*}{(b)} 
		&Vollath$\uparrow$ & 0.2542 & 0.1863 & 0.1792 & 0.1865 & 0.1939  \\
		& Variance$\uparrow$ & 0.2526 & 0.1791 & 0.1925 & 0.1812 & 0.1945 \\
		\midrule
		\multirow{2}{*}{(c)} 
		&Vollath$\uparrow$ & 0.2364 & 0.1935 & 0.1833 & 0.1889 & 0.1977 \\
		& Variance$\uparrow$ & 0.2319 & 0.1914 & 0.1885 & 0.1879 & 0.2001  \\
		\bottomrule

	\end{tabular}
	%	}
	%	\end{center}
\end{table*} 




